Comparative study of deep learning methods for the automatic segmentation of lung, lesion and lesion type in CT scans of COVID-19 patients

Recent research on COVID-19 suggests that CT imaging provides useful information to assess disease progression and assist diagnosis, in addition to help understanding the disease. There is an increasing number of studies that propose to use deep learning to provide fast and accurate quantification of COVID-19 using chest CT scans. The main tasks of interest are the automatic segmentation of lung and lung lesions in chest CT scans of confirmed or suspected COVID-19 patients. In this study, we compare twelve deep learning algorithms using a multi-center dataset, including both open-source and in-house developed algorithms. Results show that ensembling different methods can boost the overall test set performance for lung segmentation, binary lesion segmentation and multiclass lesion segmentation, resulting in mean Dice scores of 0.982, 0.724 and 0.469, respectively. The resulting binary lesions were segmented with a mean absolute volume error of 91.3 ml. In general, the task of distinguishing different lesion types was more difficult, with a mean absolute volume difference of 152 ml and mean Dice scores of 0.369 and 0.523 for consolidation and ground glass opacity, respectively. All methods perform binary lesion segmentation with an average volume error that is better than visual assessment by human raters, suggesting these methods are mature enough for a large-scale evaluation for use in clinical practice.

==> figures/lesion_classification_con.tex <==
\begin{figure*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \includegraphics{figures/boxplots/boxplot_mc_cons_binary_dice_score.png} &  
        \includegraphics{figures/boxplots/boxplot_mc_cons_binary_volume_difference.png}
        \includegraphics{figures/boxplots/boxplot_mc_cons_binary_average_surface_distance.png} &
        \includegraphics{figures/boxplots/boxplot_mc_cons_binary_hausdorff_distance.png}
    \end{tabular}
    }
    \caption{Boxplots for consolidation}
    \label{fig:boxplots_con}
\end{figure*}

==> figures/lesion_classification_cpp.tex <==
\begin{figure*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \includegraphics{figures/boxplots/boxplot_mc_cpp_binary_dice_score.png} &  
        \includegraphics{figures/boxplots/boxplot_mc_cpp_binary_volume_difference.png}
        \includegraphics{figures/boxplots/boxplot_mc_cpp_binary_average_surface_distance.png} &
        \includegraphics{figures/boxplots/boxplot_mc_cpp_binary_hausdorff_distance.png}
    \end{tabular}
    }
    \caption{Boxplots for cpp}
    \label{fig:boxplots_cpp}
\end{figure*}

==> figures/lesion_classification_ggo.tex <==
\begin{figure*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \includegraphics{figures/boxplots/boxplot_mc_ggo_binary_dice_score.png} &  
        \includegraphics{figures/boxplots/boxplot_mc_ggo_binary_volume_difference.png}
        \includegraphics{figures/boxplots/boxplot_mc_ggo_binary_average_surface_distance.png} &
        \includegraphics{figures/boxplots/boxplot_mc_ggo_binary_hausdorff_distance.png}
    \end{tabular}
    }
    \caption{Boxplots for ggo}
    \label{fig:boxplots_ggo}
\end{figure*}

==> figures/lesion_classification_mean.tex <==
\begin{figure*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \includegraphics{figures/boxplots/boxplot_mc_mean_binary_dice_score.png} &  
        \includegraphics{figures/boxplots/boxplot_mc_mean_binary_volume_difference.png}
        \includegraphics{figures/boxplots/boxplot_mc_mean_binary_average_surface_distance.png} &
        \includegraphics{figures/boxplots/boxplot_mc_mean_binary_hausdorff_distance.png}
    \end{tabular}
    }
    \caption{Boxplots for mean of classes}
    \label{fig:boxplots_mean}
\end{figure*}

==> figures/lesion_segmentation_binall.tex <==
\begin{figure*}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \includegraphics{figures/boxplots/boxplot_bin_binall_binary_dice_score.png} &  
        \includegraphics{figures/boxplots/boxplot_bin_binall_binary_volume_difference.png}
        \includegraphics{figures/boxplots/boxplot_bin_binall_binary_average_surface_distance.png} &
        \includegraphics{figures/boxplots/boxplot_bin_binall_binary_hausdorff_distance.png}
    \end{tabular}
    }
    \caption{Boxplots for binary}
    \label{fig:boxplots_binary}
\end{figure*}

==> figures/master_qualitative_bin.tex <==
\begin{figure*}[htb]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYYY}

        & CT &   WASS &     2DS &     UNWM &   CTA & CENET & InfNet  &   MAJ \\
        
        \rotatebox{90}{\hspace{20pt} IQR25} &
        \includegraphics[width=\linewidth]{figures/qualitative/binary/ct_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/WASS_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/2DS_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/UNWM_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/CTA_IQR75.png} & 
        \includegraphics[width=\linewidth]{figures/qualitative/binary/CENet_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/InfNt_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/MAJ_IQR75.png} \\ 
        
        \rotatebox{90}{\hspace{20pt} MEDIAN} &
        \includegraphics[width=\linewidth]{figures/qualitative/binary/ct_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/WASS_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/2DS_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/UNWM_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/CTA_MEDIAN.png} & 
        \includegraphics[width=\linewidth]{figures/qualitative/binary/CENet_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/InfNt_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/MAJ_MEDIAN.png} \\ 
        
        \rotatebox{90}{\hspace{20pt} IQR75} &
        \includegraphics[width=\linewidth]{figures/qualitative/binary/ct_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/WASS_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/2DS_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/UNWM_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/CTA_IQR25.png} &
        \includegraphics[width=\linewidth]{figures/qualitative/binary/CENet_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/InfNt_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/binary/MAJ_IQR25.png} \\ 
        

    \end{tabularx}
    }
        \caption{A qualitative evaluation of the resulting predictions for lesion segmentation on the validation set from each method (columns, from left to right: original CT, and predictions from WASS, 2DS, BBB, 2Dcta and MAJ). The predicted delineations are obtained after thresholding at 0.5 and each image is overlayed with the manual ground truth in red. The three rows are slices from different CT scans for which the dice score is respectively the median, first and third quartile value. The invididual slice has the median dice score among slices in that CT scan.}
    \label{fig:qualitative_master_bin}
\end{figure*}


==> figures/master_qualitative_lungs.tex <==
\begin{figure*}[htb]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYYY}

        & CT & DMLo    &  JoHof    & UNWM   & DMLu  & CTA   & WASS  & MAJ   \\

        \rotatebox{90}{\hspace{20pt} IQR25} &
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/ct_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/DMLo_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/JoHof_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/UNWM_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/DMLu_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/CTA_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/WASS_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/MAJ_IQR25.png} \\ 
        
        \rotatebox{90}{\hspace{20pt} MEDIAN} &
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/ct_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/DMLo_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/JoHof_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/UNWM_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/DMLu_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/CTA_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/WASS_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/MAJ_MEDIAN.png} \\ 
        
        \rotatebox{90}{\hspace{20pt} IQR75} &
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/ct_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/DMLo_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/JoHof_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/UNWM_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/DMLu_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/CTA_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/WASS_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative/lungs/MAJ_IQR75.png} \\ 
        

    \end{tabularx}
    }
        \caption{A qualitative evaluation of the resulting predictions for lung segmentation on the validation set from each method (columns, from left to right: original CT, and predictions from DMLo, JoHof, UNWM, DMLu, CTA, WASS and MAJ). The predicted delineations are obtained after thresholding at 0.5 and each image is overlayed with the manual ground truth in red. The three rows are slices from different CT scans for which the dice score is respectively the median, first and third quartile value. The invididual slice has the median dice score among slices in that CT scan.}
    \label{fig:qualitative_master_lungs}
\end{figure*}


==> figures/master_qualitative_mc_testset.tex <==
\begin{figure*}[htb]
    \centering
    \resizebox*{\linewidth}{!}{
    
    \def\arraystretch{0}
    \setlength{\tabcolsep}{0pt}
    \begin{tabularx}{\linewidth}{l @{\hspace{2pt}} YYYYYYY}

        &  CT &  WASS &     UNWM &  DMmc &  2DU &  InfNt &  MAJ \\

        \rotatebox{90}{\hspace{20pt} IQR25} &
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/ct_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/WASS_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/UNWM_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/DMLC_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/2DRnx_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/InfNt_IQR75.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/MAJ_IQR75.png}   \\ 
        
        \rotatebox{90}{\hspace{20pt} MEDIAN} &
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/ct_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/WASS_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/UNWM_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/DMLC_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/2DRnx_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/InfNt_MEDIAN.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/MAJ_MEDIAN.png}   \\ 
        
        \rotatebox{90}{\hspace{20pt} IQR75} &
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/ct_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/WASS_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/UNWM_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/DMLC_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/2DRnx_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/InfNt_IQR25.png} &  
        \includegraphics[width=\linewidth]{figures/qualitative_testset/multiclass/MAJ_IQR25.png} 
        

    \end{tabularx}
    }
        \caption{A qualitative evaluation of the resulting predictions for multiclass lesion segmentation on the validation set from each method (columns, from left to right: original CT, and predictions from WASS, UNWM, DMmc, 2DRnx, InfNet and MAJ). The manual ground truth is depicted as red (CONS), green (GGO), blue (CPP) and magenta (COMB) contours on each image. The predictions are shown with the same color representation. The three rows are slices from different CT scans for which the mean dice score over the different classes is respectively the median, first and third quartile value. The invididual slice has the median dice score among slices in that CT scan.}
    \label{fig:master_qualitative_mc_testset}
\end{figure*}


==> methods/lesion_classification_MAJ.tex <==
\subsection{Majority voting}
\label{sec:lesion_classification_MAJ}
Majority voting is applied for each class separately as described in Section~\ref{sec:lung_segmentation_MAJ}.

==> methods/lesion_segmentation_MAJ.tex <==
\subsection{Majority voting}
\label{sec:lesion_segmentation_MAJ}
Majority voting is applied as described in Section~\ref{sec:lung_segmentation_MAJ} considering the following methods: CT Angel, 2DS, WASS and BBB methods (the latter two are described in the next section). 

==> methods/lung_segmentation_MAJ.tex <==
% Random vectors
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
% Vectors
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}

\subsection{Deep neural networks ensembling}
\label{sec:lung_segmentation_MAJ}
In this subsection, we discuss the role of ensembling for segmentation using deep learning.

Deep learning methods for segmentation depend on many hyperparameters.
% 
These hyperparameters include
% 
the choice of the architecture with different depths, number of layers and strategy to handle multi-scale information,
% 
the choice of the loss function,
% 
the choice of the optimizer and the optimization parameter such as the learning rate,
% 
the choice of addressing one task or several,
% 
and also the choice of the data preprocessing steps and the type of data augmentation operations used during training.

Different deep learning methods can give similarly good segmentations, but they are likely to have different biases and to make different mistakes.
In this case, the ensembling of diverse models can lead to averaging out the inconsistencies due to the hyperparameter and improve the segmentation performance and robustness.

\cite{kamnitsas2017ensembles} proposed a formalization of this problem.
% 
Let $\rvx$ and $\rvy$ two random variables corresponding to a CT scan and the corresponding segmentation.
% 
After training, a deep neural network trained for segmentation gives an approximation
$P(\rvy | \rvx; \vtheta_{\vmu}, \vmu) \approx P(\rvy | \rvx)$ of the posterior segmentation distribution, where $\vtheta_{\vmu}$ is the vector of trainable parameters of the network obtained after training, and $\vmu$ are the vector of hyperparameters that were chosen when designing the deep learning pipeline.
% 
Assuming that $P(\rvy | \rvx; \vtheta_{\vmu}, \vmu)$ is an unbiased estimator of $P(\rvy | \rvx)$, and that a set of trained networks corresponding to hyperparameters $\{\vmu_1, \ldots, \vmu_M\}$ drawn among optimal the set hyperparameter settings are available, an unbiased \textit{ensembling estimation} of $P(\rvy | \rvx)$ with reduced variance is given by:
\begin{equation}
    \frac{1}{M} \sum_{m=1}^M P(\rvy | \rvx; \vtheta_{\vmu_m}, \vmu_m) \approx P(\rvy | \rvx)
\end{equation}

In practice, the maximum-a-posteriori segmentation of the ensembling model is computed directly by applying a majority voting to every voxel of the segmentations predicted by the individual models after argmax.
% 
In case different classes obtained the same score after majority voting, the class predicted by the ensemble is chosen randomly among them.

% In order to have an upper boundary for comparing each of the individual methods against, we also calculate the ensemble of all the methods described above. Ensembling is performed by applying a majority voting strategy on the voxel-level after thresholding at $0.5$.
